Where have you been? A Study of Privacy Risk for Point-of-Interest Recommendation

As location-based services (LBS) have grown in popularity, more human mobility data has been collected. The collected data can be used to build machine learning (ML) models for LBS to enhance their performance and improve overall experience for users. However, the convenience comes with the risk of privacy leakage since this type of data might contain sensitive information related to user identities, such as home/work locations. Prior work focuses on protecting mobility data privacy during transmission or prior to release, lacking the privacy risk evaluation of mobility data-based ML models. To better understand and quantify the privacy leakage in mobility data-based ML models, we design a privacy attack suite containing data extraction and membership inference attacks tailored for point-of-interest (POI) recommendation models, one of the most widely used mobility data-based ML models. These attacks in our attack suite assume different adversary knowledge and aim to extract different types of sensitive information from mobility data, providing a holistic privacy risk assessment for POI recommendation models. Our experimental evaluation using two real-world mobility datasets demonstrates that current POI recommendation models are vulnerable to our attacks. We also present unique findings to understand what types of mobility data are more susceptible to privacy attacks. Finally, we evaluate defenses against these attacks and highlight future directions and challenges. Our attack suite is released at https://github.com/KunlinChoi/POIPrivacy.

==> otherinfo.tex <==
\begin{algorithm}[h]
\caption{Original Likelihood Ratio Attack (LiRA) \jinghuai{No need mention original}}
\label{alg:lira_ori}
\begin{algorithmic}[1]
\Require query result from the target model:$conf_{\text{obs}}$, query score from "IN" model: $conf_{\text{in}}$, query score from "OUT" model: $conf_{\text{out}}$, target input: X
\Ensure a score for membership:$\Lambda$

\State $\mu_{\text{in}} \leftarrow$ mean($conf_{\text{in}}[X]$)
\State $\mu_{\text{out}} \leftarrow$ mean($conf_{\text{out}}[X]$)
\State $\sigma_{\text{in}}^2 \leftarrow$ var($conf_{\text{in}}$)
\State $\sigma_{\text{out}}^2 \leftarrow$ var($conf_{\text{out}}$)
\State\Return $\Lambda = \frac{p(conf_{\text{obs}} | N(\mu_{\text{in}},\sigma_{\text{in}}^2))}{p(conf_{\text{obs}} | N(\mu_{\text{out}},\sigma_{\text{out}}^2))}$
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[h]
\caption{Common Location Extraction Attack -- math version\jianfeng{This algorithm description is *very* unclear and misleading}}
\label{alg:common_point}
\begin{algorithmic}[1]
\Require victim model:$f_{\theta}$, target user ID: $u$, selection size:$k$, query mumber:$q$,query timestamp:$t$, random location selection algorithm: $\textsc{RandomLocation}$
\Ensure  Top-k locations and their confidence score: AC %

\State AC $\leftarrow \emptyset$ %
\For{0 to q-1}
    \State $l \leftarrow$ Randomly sample a location $l \in$ \locspace %
    \State AC $\gets$ AC $\cup$ $f_{\theta} \big(u, \{(l, t)\} \big)$
\EndFor
\State \Return AC $\gets \argmax_k$(AC) \todo{\jinghuai{output does not match your declared output}}
\end{algorithmic}
\end{algorithm}




\begin{table*}[!htbp]\renewcommand{\arraystretch}{1.2}
\fontsize{8.5}{8.5}\selectfont
\centering
\caption{Notations}
\setlength{\tabcolsep}{1mm}
{
\begin{tabularx}{\textwidth}{c|p{11cm}}

\midrule
\multicolumn{1}{c|}{\textbf{Notation}} & \multicolumn{1}{c}{\textbf{\centering Explanation}} \\
\midrule

\targetmodel$(*)$   & The victim DNN model for next POI recommendation    \\ \midrule
\multirow{2}{*}{\centering $(\uid, \tim, \loc)$} & Indicates a check-in event, where $Uid$ is an unique user id, $tim$ and $loc$ represent the time and location of the given check-in event \zhiqing{maybe use t or time to replace tim, not sure about this part}                                                \\\midrule
$\traj_n$          & A trajectory consists of $n$ location points {[}$loc_1, \cdots, loc_n${]}                                                                                                                 \\\midrule
\locspace         & The search space of location points,  which covers all the $loc$ that appear in the users' check-ins.                                                                                     \\ \midrule
\multirow{2}{*}{\centering \trajspace}        & The space of all possible $Traj_n$ in the dataset, which is the set of all possible sequences formed by $n$ loc $\in R_{loc}$.                                                            \\\midrule
\multirow{2}{*}{\centering $\prediction_k$}          & Top-$k$ prediction results for Common Location Extraction Attack of produced by the victim recommendation model ($f_{\theta}(*)$)\                                                          \\\midrule
\yhat      & The probability of being the common location for common location extraction attack   \\\midrule                                                                                           
\y            & The percentage of the most common location for a user in the training dataset   \\\midrule                                                                                              
\multirow{2}{*}{\centering $\exposure$}       & The exposure score for a given trajectory defined in \cite{236216}, which is a metric that quantifies the memorization of the model toward a specific training sequences \\ \midrule
$\beta$            & The beam width for the raining data extraction attack          \\  \midrule                                                                                                 
$\candidate$            & Candidate to keep for beam search    \\ \midrule 
$\shadownumber$      & Number of shadow models used in the membership inference attack.       \\        \midrule                                            
$\train$               & The training process for shadow model                                           \\ \midrule 
$\confidence$            & The continuous confidence score for the model output\\\midrule 
$\Lambda$            & The probably output of the null-hypothesis indicating if the trajectory is member or not\\ \midrule 

\end{tabularx}
}
\label{notation}
\end{table*}





\begin{algorithm}[h]
\caption{Training Trajectory Extraction Attack \jianfeng{This algorithm description is *very* unclear and misleading}}
\label{alg:TrainingTraj}
\begin{algorithmic}[1]
\Require Target User ID: $u$, starting location:$l_0$, target extraction length:$n$, beam width: $\beta$, 
\Ensure A beam for possible extraction results $B$
\State $ppl_{init}$,$t$ $\leftarrow 0,0.5$ 
\State $B \leftarrow$ $\emptyset$
\For{$0 \text{ to } \beta$}
    \State $B \gets B \cup$ ($l_0$,$ppl_{init}$)
\EndFor \Comment{Initialize Beam}

\For{$i \leftarrow 0 \text{ to } n$}
    \State $ppl_{new} \gets \emptyset$
    \For {($\{(l_0, t)..(l_i, t))\}$,$ppl$) $\text{ in } B$}
        \State output $\leftarrow f_{\theta}(u, \{(l_0, t)..(l_i, t))\}$ 
        \For {$l$ in $\mathcal{L}$}
            \State $x \gets \{(l_0, t)..(l_i, t),(l,t))\}$
            \State $ppl_{new}$= $ppl_{new} \cup $($x$,(ppl $- \log_2(\mathrm{output}$[$l$])))
        \EndFor
    \EndFor
    \State $B = \argmin_{\beta \in ppl_{new}}(\text{ppl}(\beta))$
    \State \kunlin{$B$ =$\{ j \in \{1, \ldots, n\} \mid \text{{ppl}}_j < \text{{ppl}}_\beta \text{{ for }} (x, \text{{ppl}}) \in \text{{ppl}}_{\text{{new}}} \}$.}

\EndFor
\State \Return $B$
\end{algorithmic}
\end{algorithm}


